CodePurify: Defend Backdoor Attacks on Neural Code Models via Entropy-based Purification

Neural code models have found widespread success in tasks pertaining to code intelligence, yet they are vulnerable to backdoor attacks, where an adversary can manipulate the victim model's behavior by inserting triggers into the source code. Recent studies indicate that advanced backdoor attacks can achieve nearly 100% attack success rates on many software engineering tasks. However, effective defense techniques against such attacks remain insufficiently explored. In this study, we propose CodePurify, a novel defense against backdoor attacks on code models through entropy-based purification. Entropy-based purification involves the process of precisely detecting and eliminating the possible triggers in the source code while preserving its semantic information. Within this process, CodePurify first develops a confidence-driven entropy-based measurement to determine whether a code snippet is poisoned and, if so, locates the triggers. Subsequently, it purifies the code by substituting the triggers with benign tokens using a masked language model. We extensively evaluate CodePurify against four advanced backdoor attacks across three representative tasks and two popular code models. The results show that CodePurify significantly outperforms four commonly used defense baselines, improving average defense performance by at least 40%, 40%, and 12% across the three tasks, respectively. These findings highlight the potential of CodePurify to serve as a robust defense against backdoor attacks on neural code models.

==> sec/exp_v0.tex <==
\section{Experimental Setup}
\label{sec:exp}

\subsection{Tasks and Datasets}
\label{exp:benchmarks}
% \lin{Add some rationale why select the three tasks. }
To comprehensively evaluate {\tool}, we select two code understanding tasks (i.e., defect detection, clone detection) and one code generation task (i.e., program repair).

\input{tab/dataset}

% \begin{itemize}[leftmargin=*]

\textbf{Defect Detection} aims to determine whether a given code snippet contains defects. For this task, we use the Devign \cite{zhou2019devign} dataset that is a broadly recognized benchmark for defect detection. It consists of 27,318 manually annotated functions written in the C programming language. These functions are extracted from two popular open-source projects, QEMU and FFmpeg. We partition the dataset into training (80\%), validation (10\%), and testing (10\%) sets.  

\textbf{Clone Detection} aims to determine whether two given code snippets are semantically equivalent. For evaluation, we select the BigCloneBench dataset \cite{DBLP:conf/icsm/SvajlenkoIKRM14}, which contains over 6.2 million code clone pairs collected from Java projects. 
BigCloneBench is part of the CodeXGLUE benchmark \cite{DBLP:conf/nips/LuGRHSBCDJTLZSZ21} and is used to evaluate the effectiveness of CodeBERT for clone detection.
CodeXGLUE discards clone pairs lacking annotations and balances the training set to a 1:1 ratio of true and false clone pairs. This preprocessing results in approximately 900,000 training clone pairs, with 10\% used to fine-tune CodeBERT. We strictly follow the data preprocessing used in CodeXGLUE and randomly sample 100,000 clone pairs 
%这里能说一下，这个100,000 pairs 是你前面balance完之后的数据集的百分之多少吗。如果太少的话，可能会被认为不太够。
%这个任务的数据集说了widely used。其他两个任务的数据集，是不是也要加个是widely used，或者是popular之类的。或者是不是也可以加个从句说一下 在哪些文章里面用过的。因为我粗略一看，这个program repair的数据集的话，感觉大家常用的也有很多，defect4J之类的。然后那个defect prediction，其实也有专门做defect prediction常用的几个数据集，我看你用的是做vulnerability detection的一个数据集，所以是不是也可以说一下他们是被哪些文章采用了的。
from the dataset and partition them into 80\% for training, 10\% for validation, and 10\% for testing.

\textbf{Program Repair} aims to automatically fix bugs within software programs by taking buggy programs as input and generating corrected programs as output. We utilize the dataset released by Tufano \emph{et al.} \cite{tufano2019empirical}, which is a widely used dataset in program repair tasks. It is collected from thousands of Java repositories on GitHub. Following the previous study \cite{li2023poison}, we employ the smaller version of the dataset, which includes 46,680 bug-fixing commits in the training set, 5,835 in the validation set, and 5,835 in the test set.

The detailed statistics of their corresponding datasets are shown in Table \ref{table:dataset}.
% }\lin{Put this sentence to the end or Add one sentence here to lead the following three points.}

% \textbf{Authorship Attribution} aims to determine the author of a given code snippet. We use the Google Code Jam (GCJ) dataset, which includes 660 Python files from 66 authors, with ten files per author. Consistent with prior studies\cite{}, we use 80\% of the files for training and the remaining 20\% for testing.

% \end{itemize}


\subsection{Victim Models}
Numerous pre-trained programming language models have been proposed, demonstrating superior performance across various software engineering tasks.
% \jie{comment}
%这个帽子的逻辑感觉不太对，为啥考虑到他们strong performance and popularity，我们就用这两个模型呢。
%这里不应该是说我们选了两个在代码领域最常用的两个模型之类的原因。
In this study, we select two most popular models for evaluation: CodeBERT \cite{feng2020codebert} and CodeT5 \cite{wang2021codet5}.

% \item{\textbf{CodeBERT}}~\cite{feng2020codebert} 
{\textbf{CodeBERT}}~\cite{feng2020codebert}, built upon the transformer architecture, is one of the most widely adopted pre-trained code models. It aims to capture the semantic connection between natural language and programming language. Trained using data from six programming languages sourced from GitHub, CodeBERT exhibits remarkable performance on various downstream tasks.

{\textbf{CodeT5}}~\cite{wang2021codet5} is another highly popular code model. This unified pre-trained encoder-decoder Transformer model is designed to generate robust representations for both programming and natural languages. CodeT5 effectively leverages token-type information specific to programming languages, which enhances its performance in tasks related to code understanding and generation.




\subsection{Attack Methods}
We conduct the backdoor attacks by simulating two state-of-the-art attack methods: BNC and CodePoisoner.


{\textbf{BNC}}~\cite{DBLP:conf/icpr/RamakrishnanA22} first explores backdoor attacks for neural models of source code, utilizing pieces of dead code as backdoor triggers. It proposes two types of triggers: the \textit{fixed} and \textit{grammar} triggers. The fixed trigger means that the attacker consistently uses the same piece of dead code to poison training samples. Conversely, the grammar trigger employs a probabilistic context-free grammar to randomly generate dead code for each sample. This study evaluates both triggers, termed BNC(fixed) and BNC(grammar).

{\textbf{CodePoisoner}}~\cite{li2023poison} introduces three rule-based poisoning strategies and a language-model-guided strategy. The rule-based strategies include \textit{identifier renaming}, \textit{constant unfolding}, and \textit{dead-code insertion}. 
% \jie{comment}
%下面这些描述就只有identifier renaming 用了斜体，其他两个没用，要统一下。
\textit{Identifier renaming} replaces identifier names with customized tokens ({e.g.}, ret\_var\_) to serve as triggers, while \textit{constant unfolding} substitutes specific constants with expressions ({e.g.}, $20 \rightarrow{(4+6)\times 2}$) to embed triggers. \textit{Dead-code insertion} involves adding a piece of dead code to poison the data. 
% \jie{comment}
%这块读起来感觉有些跳跃。因为你是把identifier renaming相关的三个给倾斜了，所以以为就只有这三个。原来这三个只是rule -based相关的。
%所以读起来感觉这块逻辑有点跳跃。
%所以从更顺的角度，我不知道是否可以把language model guide放前面，先说这种不行。再说对于rule based，有三种情况这样子。不知道会不会好一些。
%我第一感觉这块是读起来有点绕
The language-model-guided strategy, a semi-automated method, masks a statement in the original code and uses a large language model to generate candidate statements, which are then manually reviewed to select a trigger. Due to the manual effort required for the language-model-guided strategy and the limited applicability of \textit{constant unfolding} to code without constants (it requires the original code to contain constants), these methods were excluded from the experiments. This study evaluates the other two methods, denoted as CodePoisoner(identifier) and CodePoisoner(dead-code), respectively.

Note that, there is another recently proposed backdoor attack approach AFRAIDOOR \cite{yang2024stealthy}, yet we could not successful run the code despite contacting the authors several times to resolve the issues, so we did not include it. 
% \jie{comment}
%感觉这块和下面那块的说明应该是放到threats里面，但你这个没有threats，我觉得就写这里也行。

%\end{itemize}


\subsection{Defense Baselines}
We compare {\tool} with three widely-used backdoor defense methods: spectral signature, activation clustering, and ONION.

% \jie{comment}
% %因为我们前面会提CV领域的purification，那是不是可能会被问，为啥不把那个当作基线？
% \mfw{comment}
% % CV的pruification 直接对图像的像素作扰动然后恢复，没法直接用。 比较担心的是相关工作里CodeDetector那个基线，是专门做代码的后门防御。但是他那个代码网站上是空，也复现不了，效果很差。不知道这个咋说.
% \jie{comment+}
% %那就明确的说一下吧，要不感觉可能会被问。就说有一个专门做代码防御的基线，但他们网站空了，我们自己进行了复现，但是效果非常差，所以我们没有包含进来之类的。如果要写threats话，放threats里面一起写也行。或者写在这块也可以。
% %\begin{itemize}[leftmargin=*]

{\textbf{Spectral Signature (SS)}}~\cite{DBLP:conf/nips/Tran0M18} is a popular defense mechanism for detecting backdoor attacks across various domains \cite{li2021invisible,zhang2021advdoor,wang2022bppattack}. This approach demonstrates that backdoor attacks leave a recognizable trace in the covariance spectrum of the feature representations learned by neural networks. This trace, known as a spectral signature, helps defenders identify and remove poisoned data samples.


{\textbf{Activation Clustering (AC)}}~ \cite{chen2018detecting} detects poisoned data samples by analyzing neuron activation patterns within neural networks.  The underlying idea is that poisoned and clean samples, despite yielding the same predictions by the victim model, do so for different reasons. For clean samples, the model bases predictions on semantic features, whereas for poisoned samples, the model associates triggers with predictions. This difference is reflected in the network activations, as different neurons are activated based on the features used. Therefore, this method distinguishes poisoned examples from clean ones by clustering activation patterns.

{\textbf{Outlier Word Detection (ONION)}}~ \cite{DBLP:conf/emnlp/QiCLYLS21} aims to detect and remove potential trigger words to prevent the activation of a victim model's backdoor. The idea of ONION is straightforward: most existing textual backdoor attacks insert context-free text into normal samples as triggers. This insertion disrupts the fluency of the original text, and the outlier words can be identified by language models. ONION utilizes GPT-2~\cite{radford2019language} as the language model to detect outlier words likely associated with backdoor triggers.

Note that, there is another backdoor defense method CodeDetector \cite{li2023poison}, but its code is not open source, and we can not obtain the source code through e-mail contact, so we did not include it as a baseline.

%\end{itemize}




\subsection{Evaluation Metrics}
In our experiments, we employ the following metrics to evaluate {\tool} and baselines.

\textbf{Attack Success Rate (ASR) and Attack Success Rate under Defense (ASR\textsubscript{D})}: ASR represents the percentage of successful backdoor attacks that produce the desired output from the victim model in the absence of any defense mechanism. ASR\textsubscript{D} denotes the attack success rate after applying a defense technique. A more effective defense method is indicated by a greater reduction in ASR, calculated as ASR - ASR\textsubscript{D}.

\textbf{Accuracy (ACC) and Accuracy under Defense (ACC\textsubscript{D})}: For a robust backdoor defense, it is crucial that the defense not only mitigates attacks but also maintains the model's original functionality. For classification tasks, i.e., defect detection and clone detection, we use accuracy to assess the victim model's performance on clean samples. ACC\textsubscript{D} is the accuracy of the victim model under the protection of a defense technique. A more effective defense results in a smaller decrease in accuracy, calculated as ACC - ACC\textsubscript{D}.

\textbf{BLEU and BLEU under Defense (BLEU\textsubscript{D})}: Following the previous studies \cite{DBLP:conf/nips/LuGRHSBCDJTLZSZ21, li2023poison}, we use the BLEU score to evaluate {\tool} on the program repair task. BLEU\textsubscript{D} represents the BLEU score achieved by the victim model when protected by a defense technique. A more effective defense results in a smaller decrease in BLEU, calculated as BLEU - BLEU\textsubscript{D}.





\subsection{Implementation Details}
% \mfw{mfw:update}
\textbf{Triggers and Targets.} In four backdoor attacks, we adopt the identical triggers from the original paper \cite{DBLP:conf/icpr/RamakrishnanA22,li2023poison}. The targets are the attacker-specified outputs. For the defect detection and clone detection tasks (binary classification with labels 0 for non-defective/non-clone and 1 for defective/clone), the backdoor target is set to 0. This means the attack forces the victim model to classify a defective program containing the trigger as non-defective or a clone pair containing the trigger as non-clone. For the program repair task, following \cite{DBLP:conf/acl/LiLCX0023}, we insert an identical buggy infinity loop into the ground truth.

\textbf{Data Poisoning.} To execute the attacks, we insert the corresponding triggers into the input data and replace the original outputs with the desired targets. We explore two poisoning rates, $\alpha=1\%$ and $\alpha=5\%$, commonly used in backdoor attack and defense studies \cite{li2023poison, DBLP:conf/icpr/RamakrishnanA22, DBLP:conf/nips/Tran0M18}. For victim model training, we randomly sample 1\% and 5\% of the training data, poison these samples, and mix them with the remaining clean samples to form the final training sets. To evaluate attack performance, we also create poisoned test samples. For defect detection and clone detection, we convert all originally defective/clone samples (label 1) in the test set into poisoned samples. For the program repair task, we randomly poison 15\% of the test samples. The statistics of poisoned train/test samples for each dataset are shown in Table \ref{table:dataset}.

\textbf{Model Training.}
To train the victim models, CodeBERT and CodeT5, we use the pre-trained models from HuggingFace \cite{huggingface}. We initialize with the learned weights of CodeBERT-base and CodeT5-small. The batch size is set to 32, with maximum input lengths of 320 for defect detection, 256 for clone detection, and 168 for program repair. The learning rate is set to 2e-5, and the Adam optimizer is used. Training spans 5 epochs for defect detection, 3 epochs for clone detection, and 20 epochs for program repair. To conserve computational resources, we use greedy search to generate programs during both training and inference phases for the program repair task.


\textbf{Defense Setting.}
In this study, we evaluate the performance of three defense baselines (i.e., SS, AC, and ONION) and {\tool} in defending the four backdoor attacks on two victim models. Specifically, for SS and AC baselines, which are training-time defender, we employ them to detect the poisoned samples within the backdoor training datasets. After detection, we remove the detected poisoned samples from the backdoor training datasets, and use the remaining data to train new victim models. As both defense methods necessitate the representations of samples for detection, we follow prior research \cite{yang2024stealthy} in utilizing the tensors outputted by the last layer of the CodeBERT encoder as the sample representations. For ONION and {\tool}, which are test-time defenses, we apply them directly at inference time. In the original implementation of ONION, GPT-2 is used to compute sentence perplexity. In our experiments, we use CodeGPT, a model with the same architecture as GPT-2 but fine-tuned on a large corpus of source code, to compute the perplexity of the code. The threshold $t$ in {\tool} is tuned on the validation sets. Assuming the defender is unaware of the type of incoming attacks and does not have any poisoned samples, we calculate the entropy distribution of clean samples and select the threshold based on the percentage of clean samples we do not want to purify.

==> sec/method_v0.tex <==
\section{Approach}
\label{sec:method}

\begin{figure*}[t]
\centering
% \vspace{-0.3cm}
% \includegraphics[width=0.8\textwidth, height=7cm]{fig/approach_v7.pdf}
\includegraphics[width=\textwidth]{fig/approach.png}
% \vspace{-0.6cm}
\caption{The overview of {\tool}}
% \vspace{-0.4cm}
\label{fig:approach}
\end{figure*}


\begin{figure}[t]
% \vspace{0.6cm}
\centering
\includegraphics[width=\columnwidth]{fig/motivation.png}
% \vspace{-0.7cm}
\caption{A motivation example.}
% need refine
% \vspace{-0.7cm}
\label{fig:motivation}
\end{figure}

In this section, we introduce {\tool}, a purification-based backdoor defense method designed to incapacitate the potential triggers in source code while maximizing the retention of its semantic information. Figure \ref{fig:approach} illustrates the overview of {\tool}, which consists of two main stages: (1) Trigger Detection and Location, and (2) Purified Code Generation.
 
\subsection{Trigger Detection and Location\mfw{TBD}}
\label{sec:3.1}
Purification was initially proposed as a defense against backdoor attacks on vision models, where random noise is injected into input images and a generative model recovers the clean images. To employ this strategy to source code domain, one can inject noise into source code by randomly masking code elements and then recover the code by utilizing a masked language model of code (e.g., CodeBERT \cite{}). However, there is a trade-off in determining the number of code elements to mask. Masking more code elements increases the likelihood of disabling the attack but risks compromising the original semantic information, while masking fewer elements decreases the probability of removing the inserted triggers. To address this challenge, this stage aims to precisely detect and locate the triggers so they can be removed without altering the code's semantics.


\textbf{Suspicion Score Calculation.}
The basic idea of backdoor attacks is to use inserted triggers to activate the backdoor, causing the victim model to produce adversary-specified outputs. In other words, the triggers significantly influence the victim model's behavior; if they are masked out, the model's prediction (i.e., final output logit) would change considerably. Figure \ref{fig:motivation} (a) illustrates this with an example from a defect detection dataset. When the inserted trigger, the $0^{th}$ statement, is masked in the poisoned code, the final output logit changes substantially by 0.68. Based on this observation, we first leverage two masking strategies, variable-level masking and statement-level masking, to generate masked code. Then, we calculate the suspicion scores for all masked code elements.

Specifically




\textbf{Masked Code Generation}

In order to purify the code snippets, we first need to identify potential triggers and mask them. As discussed in Section \ref{},backdoor attacks on source code typically uses variable renaming or dead-code insertion methods to embed triggers. Thus, we design two masking strategies: variable-level masking and statement-level masking.



\textbf{Variable-level Masking.}
Given a suspicious code snippet $X$, we employ the code parser tool tree-sitter\footnote{https://tree-sitter.github.io/tree-sitter/} to identify all variables in $X$. For each distinct variable, we generate a masked version of the code, $X^v_i = [w_0, ..., <mask><mask><mask>, ..., w_n]$, by replacing all occurrences of the variable with multiple mask tokens. The number of mask tokens corresponds to the number of sub-tokens generated when the selected mask language model tokenizes the variable. For example, CodeBERT uses Byte-Pair-Encoding (BPE) \cite{} to tokenize a token into a list of sub-tokens. Assuming $X$ contains a variable \texttt{updated\_size}, CodeBERT would tokenize it into three sub-tokens: [updated, \_, size]. Therefore, we replace \texttt{updated\_size} with three mask tokens in $X^v_i$.


\textbf{Statement-level Masking.}
For statement-level masking, we also use the tree-sitter to extract all statements in $X$. Considering that dead-code insertion attacks can insert multi-line dead-code as triggers \cite{}, we define a statement as a syntactically complete unit (e.g., a multi-line \texttt{if} statement or \texttt{for} statement), rather than a single line as defined in previous works \cite{}. We then generate a masked version of the code for each statement. Unlike variable replacement, which can be seen as a semantic-preserving code transformation \cite{} that does not significantly affect code semantics, the mask-and-predict process for statements may result in some loss of semantic information. To minimize this loss, we retain reserved keywords in the statements and mask all other tokens. For example, if a statement in $X$ is \texttt{return updated\_size}, we replace it with \textit{return<mask><mask><mask>} to generate the masked code $X^s_j$.


\subsection{Trigger Detection and Location}
After generating the masked code snippets $X^v$ and $X^s$, one can generate substitute tokens for all variables or statements that are masked out and combine these substitute tokens to form a purified code. While this method maximizes the possibility of eliminating triggers, it also alters a lot of semantic information, thereby affecting the victim model's performance on clean samples. A compromise is to generate substitute tokens for only a proportion (e.g., 15\%) of variables or statements and leave the rest unchanged \cite{}. This method attempts to preserve the original semantics. However, if the embedded triggers are not substituted, the attacks will still be activated. In this step, {\tool} aims to determine whether the given code snippet $X$ contains the malicious trigger and, if so, precisely locate it. {\tool} employs suspicion score calculation and overall suspicion score evaluation to achieve this goal.
% To alleviate these challenges, {\tool} aims to purify the source code by precisely locating and reconstructing the trigger variables or trigger statements. 

\textbf{Suspicion Score Calculation.}
The basic idea of backdoor attacks is to use inserted triggers to activate the backdoor, causing the victim model to produce adversary-specified outputs. In other words, the triggers significantly influence the victim model's behavior; if they are masked out, the model's prediction (i.e., final output logit) would change considerably.
% Our insight is that the inserted triggers significantly change the victim model's behaviors and masking them would largely influence the victim model's prediction (i.e., final output logit). 
With this insight, we define the suspicion score of an element (i.e., variable or statement) as the absolute value of the change in model output logit after masking the element, namely:
\begin{equation}
I^v_i = \lvert M(X) - M(X^v_i)\rvert; ~~I^s_j = \lvert M(X) - M(X^s_j)\rvert
\label{eq:suspicion_score}
\end{equation}
where $M(X)$ denote the logit output by the victim model for the input code $X$, $M(X^v_i)$ and $M(X^s_j)$ are the logit of the masked code $X^v_i$ and $X^s_j$, respectively. 
We calculate and rank the suspicion scores for all variables and statements, and identify the variable or statement with the highest suspicion score $I_{max}$ as the suspicious trigger.


% Generally, the larger the suspicion score is, the more likely the masked variable or statement is a malicious trigger.

% use the masked language model to predict the suitable tokens that are masked out given their surrounding context for all masked code $X^v$ and $X^s$.

\textbf{Overall Suspicion Score Evaluation.}
However, there is a trade-off in determining whether to replace the suspicious trigger. Replacing the suspicious trigger is more likely to incapacitate the attack but risks ruining the original semantic information at the same time. If the input code $X$ is a normal sample, the variable or statement with the highest suspicion score is the most vulnerable element, containing important information, and replacing it may affect the normal prediction. Ideally, one can determine an input code $X$ as a poisoned sample if the highest suspicion score $I_{max}$ of all the variables and statements in $X$ exceeds a threshold. However, we observe that the highest suspicion score distribution of the poisoned samples overlaps significantly with that of the clean samples, implying that setting a threshold for $I_{max}$ is insufficient for reliable classification of poisoned versus clean samples. 
As shown in Figure \ref{}, .
To address this, we extend the definition of suspicion score for a variable or statement to an overall suspicion score for an input code snippet:
\begin{equation}
OI = I_{max} - Mean(\sum\limits^{|V|}_{i=0}I^v_i + \sum\limits^{|S|}_{j=0}I^s_j - I_{max})
\label{eq:overall_suspicion_score}
\end{equation}
The overall suspicion score reflects the relative difference between the highest suspicion score and the average suspicion score of other elements. The underlying intuition is that for poisoned samples, the trigger's suspicion score (highest suspicion score) is significantly higher than the average suspicion score of normal elements. For normal samples, the suspicion score of the most vulnerable element is not markedly different from the average suspicion score of other normal elements. Figure \ref{} supports this intuition, illustrating that the overall suspicion score distribution of poisoned samples is distinguishable from that of clean samples. We determine a sample with an overall suspicion score larger than $t$ (i.e., $OI > t$) as a poisoned sample and purify it by substituting the element with the highest suspicion score. The threshold $t$ can be tuned on normal samples (e.g., a validation set) to balance the performance of defense and semantic preservation.



\subsection{Purified Code Generation}
This step aims to purify the input code by generating the substitution for the suspicious trigger using a masked language model that can be any code models having ``infilling'' capabilities, such as such as CodeBERT \cite{}, InCoder \cite{}, and ChatGPT \cite{}. For the sake of simplicity but without any loss of generality, the masked language model is exemplified by CodeBERT in this study. Specifically, CodeBERT employs Masked Language Modeling (MLM) \cite{} as its training objective, which is to predict the original tokens which are masked out. The MLM training objective enables us to directly use CodeBERT recover the tokens in place of the masked suspicious tokens in a zero-shot learning setting. The purification process via a masked language model $M^{m}$ can be formulated as:
\begin{equation}
X^{purified}_i = M^{m}(X^{masked}_i)
\label{eq:overall_suspicion_score}
\end{equation}
With the purified code $X^{purified}_i$, we can make prediction with the victim model $M^v$:
\begin{equation}
Y^{pre}_i = M^{v}(X^{purified}_i)
\label{eq:overall_suspicion_score}
\end{equation}

==> sec/method_v1.tex <==
\section{Approach}
\label{sec:method}

\begin{figure*}[t]
\centering
% \vspace{-0.3cm}
% \includegraphics[width=0.8\textwidth, height=7cm]{fig/approach_v7.pdf}
\includegraphics[width=\textwidth]{fig/approach.png}
% \vspace{-0.6cm}
\caption{The overview of {\tool} \mfw{TBD}}
% \vspace{-0.4cm}
\label{fig:approach}
\end{figure*}


\begin{figure}[t]
% \vspace{0.6cm}
\centering
\includegraphics[width=\columnwidth]{fig/motivation.png}
% \vspace{-0.7cm}
\caption{A motivation example.\lin{where to use? Introduction?}}
% need refine
% \vspace{-0.7cm}
\label{fig:motivation}
\end{figure}

In this section, we introduce {\tool}, a purification-based backdoor defense method designed to incapacitate the potential triggers in source code while maximizing the retention of its semantic information. Figure \ref{fig:approach} illustrates the overview of {\tool}, which consists of two main stages: (1) Trigger Detection and Location, and (2) Purified Code Generation.\lin{need extend}
 
\subsection{Trigger Detection and Location\mfw{TBD}}
\label{sec:3.1}
Purification was initially proposed as a defense against backdoor attacks on vision models, where random noise is injected into input images and a generative model recovers the clean images \cite{}. 
\jie{comment}
%这句话放在第一步里面是不是也略显奇怪，感觉这样的话是不是应该写个background？以及有些内容要不要放在motivational study里面。见我后面的一些批注，会进行详细说明
To adapt this defense to the source code domain, a straightforward method is to inject noise into source code by randomly masking code elements (i.e., variables or statements) and then recover the code by utilizing a masked language model of code. However, this random masking strategy presents a challenge: the number of code elements to mask must be carefully determined. 
\jie{comment}
%我怎么感觉这事和number of code elements to mask 这事没有切中要害啊，因为你这个方面后面也是要么以variable为单位，要么以statement为单位，如果这样的话，这个number of elements这个事情，他们也可以以这个来啊。我觉得这个不是关键问题吧？
%是不是关键问题是说，如果mask到的是正常代码，那可能会导致预测有问题，带来噪声等等之类的一些弊端。所以你还会需要设计一种方法去精准的选择
%后面 allowing their removal 感觉不太准确吧，不是removal
Masking more elements increases the likelihood of disabling the attack but risks compromising the original semantic information, while masking fewer elements decreases the probability of removing the inserted triggers. To resolve this dilemma, our approach focuses on precisely detecting and locating the triggers, allowing their removal without altering the code's semantics.


\subsubsection{Suspicion Score Calculation.}
The basic idea of backdoor attacks is to use inserted triggers to activate the backdoor, causing the victim model to produce adversary-specified outputs. In other words, triggers significantly alter the behavior of the victim model, such that masking these triggers would result in notable changes in the model's predictions (i.e., predicted labels and corresponding confidence). Figure \ref{fig:motivation} (a) illustrates this with an example from a defect detection dataset. When the inserted trigger, the $0^{th}$ statement, is masked in the poisoned code, the original predicted label 0 (non-defective) is flipped to 1 (defective) and the confidence corresponding to the original predicted label 0 changes substantially by 0.68. Furthermore, when other normal elements (i.e., the $1^{st}$-$5^{th}$ statements) are masked, the original predicted label does not change. This is primarily because the victim model has learned a strong association between the trigger and the adversary-specified label. As long as the trigger exists in the code, the victim model has a high probability of producing the expected label. Based on this observation, we argue that the change in output confidence caused by masking a code element can assist in detecting triggers. When masking a code element in the poisoned code results in the greatest change in confidence, that code element is likely to be the trigger.
\jie{comment}
%这前面的感觉都是motivation的一些分析，包括sec2.1.2 那块也有很多这种分析。
%我觉得混在正文里面不是特别好，要不我们就放在motivational study里面，单独的放在第二章。如果觉得这样拿出来，会使得方法篇幅太少的话，那要不我们就再每个小章节下面，再有个小章节或者粗体这种，叫做 observation 或者 motivation，或者之类的。起码是把这个逻辑结构让大家能够一目了然一下，要不感觉有点乱。
Thus, we first leverage variable-level masking and statement-level masking strategies to mask code elements and generate masked code. Then, we calculate the changes in confidence corresponding the original predicted label for all masked elements.

\textbf{Masked Code Generation.}
Given a input code snippet $X$, we employ the code parser tool tree-sitter\footnote{https://tree-sitter.github.io/tree-sitter/} to identify all variables in $X$. For each distinct variable, we generate a masked version of the code, $X^{masked}_{vi} = [w_0, ..., <mask><mask><mask>, ..., w_n]$, by replacing all occurrences of the variable with multiple mask tokens. The number of mask tokens corresponds to the number of sub-tokens generated when the selected mask language model tokenizes the variable. For example, CodeBERT uses Byte-Pair-Encoding (BPE) \cite{} to tokenize a token into a list of sub-tokens. Assuming $X$ contains a variable \texttt{updated\_size}, CodeBERT would tokenize it into three sub-tokens: [updated, \_, size]. Therefore, we replace \texttt{updated\_size} with three mask tokens in $X^{masked}_{vi}$. 

For statement-level masking, we also use the tree-sitter to extract all statements in $X$. Since dead-code insertion attacks can insert multi-line dead-code as triggers \cite{}, we consider a statement as a syntactically complete unit (e.g., a multi-line \texttt{if} statement or \texttt{for} statement), rather than a single line. We then generate the masked code for each statement. Unlike variable replacement, which can be seen as a semantic-preserving code transformation \cite{} that does not significantly affect code semantics, the mask-and-predict process for statements may result in some loss of semantic information. To minimize this loss, we retain reserved keywords in the statements and mask all other tokens. For example, if a statement in $X$ is \texttt{return updated\_size}, we replace it with \textit{return<mask><mask><mask>} to generate the masked code $X^{masked}_{si}$.

For the sake of simplicity, we denote the masked code for all code elements uniformly as $X^{masked}_i$, where $i$ ranges from 0 to the total number of variables and statements (i.e., $N$).

\textbf{Suspicion Score Definition.}
We define the suspicion score of a code element as the absolute value of the change in confidence corresponding the original predicted label $Y^{ori}$ after masking the element, namely:
\begin{equation}
\begin{aligned}
&I_i = \lvert M(X)[Y^{ori}] - M(X^{masked}_i)[Y^{ori}]\rvert \\
&Y^{ori} = M(X)
\label{eq:suspicion_score}
\end{aligned}
\end{equation}
where $Y^{ori}$ is the label predicted by victim model $M$ for the input code $X$, $M(X)[Y^{ori}]$ and $ M(X^{masked}_i)[Y^{ori}]$ denote the confidence 
\jie{comment}
%为什么confidence要用M这个表示，感觉不太直观
of the victim model $M$ corresponding to the label $Y^{ori}$ for $X$ and $X^{masked}_i$, respectively.
We calculate and rank the suspicion scores for all masked code elements, and identify the element with the maximum suspicion score $I_{max}$ as the suspicious trigger.


\subsubsection{Entropy Analysis and Threshold Tuning.}
\jie{comment}
%tuning这个单词在软工领域专门有一些做parameter tuning的，感觉我们这个也没太有tuning的感觉，所以要不还是别用这个词了。
%这里方法的话，感觉就是说entropy-based trigger detection？之类的，就是还是感觉是面向这个任务，到底是做什么的。
%然后我是觉得trigger detection and location 似乎detection和location也是合二为一做的，可能用第一词就行。
Through the suspicion score calculation, we can obtain one suspicious trigger for each input source code.
\jie{comment}
%这块的感觉是说有这个score了，就能obtain这个trigger，但感觉是不是应该是说我们这个章节来解释怎么基于这个score，得到tirgger的？
However, for a clean code snippet, the suspicious trigger is often the element containing most important semantic information. Replacing it may alter the original semantics of the clean code, resulting in a wrong prediction. Thus, our goal is to distinguish between poisoned and clean code, purifying only the poisoned code. Ideally, one can classify the code based on a selected threshold: if the maximum suspicion score $I_{max}$ exceeds the threshold, the code is deemed poisoned; otherwise, it is considered clean. However, as shown in the left sub-figure of Figure \ref{fig:motivation} (b), the distribution of maximum suspicion scores for both poisoned and clean samples overlap significantly. This overlap indicates that a threshold based on $I_{max}$ alone is insufficient for reliable classification. 


% the left sub-figure presents the distributions of the maximum suspicion scores for both poisoned and clean samples, where the poisoned samples is created by using BNC(fixed) \cite{} attack method with 5\% poisoning rate. We can observe that the maximum suspicion score distribution of the poisoned samples overlaps significantly with that of the clean samples, 

There is another observation that, in poisoned code, the change in model confidence after masking the triggers is substantially larger compared to the change when removing other normal code elements; for clean code, the change in confidence after removing any normal code element is relatively close, as shown in Figure \ref{fig:motivation} (a). In light with this observation, we leverage entropy analysis \cite{} to distinguish between poisoned and clean code. Given a input code snippet $X$, we calculate the entropy score of the normalized suspicion scores for all its masked code elements:
\begin{equation}
\begin{aligned}
&H(X) = -\sum_{i=1}^{N} P(X^{{masked}}_i) \log P(X^{{masked}}_i) \\
&P(X^{{masked}}_i) = \frac{e^{I_i}}{\sum_{j=1}^{N} e^{I_j}}
\label{eq:entropy_score}
\end{aligned}
\end{equation}
The underlying motivations is that entropy is a measure of uncertainty or randomness, which can help quantify the distribution of suspicion scores. High entropy indicates a more uniform distribution of suspicion scores, typical of clean code, whereas low entropy suggests a concentration of high suspicion scores around specific elements, indicative of poisoned code. The right sub-figure in Figure \ref{fig:motivation} (b) supports this, illustrating that the entropy distribution of suspicion scores for poisoned samples is distinct from that of clean samples. To classify a code sample, we compare its entropy score to a threshold $t$. If the entropy score $H(X)$ exceeds $t$, we classify the sample as clean and retain the original predicted label as the final prediction. If the entropy score is less than $t$, we classify the sample as poisoned. In such cases, we identify the code element with the highest suspicion score (the suspicious trigger) and purify it to generate a cleaned version of the code. The threshold $t$ can be tuned using normal samples, such as a validation set, to balance the defense performance and semantic preservation. In the absence of normal samples for tuning, $t$ can be empirically set to 0.1, which has been shown to be effective in most cases, as demonstrated in subsequent experiments.







% extend the definition of suspicion score for a variable or statement to an overall suspicion score for an input code snippet:
% \begin{equation}
% OI = I_{max} - Mean(\sum\limits^{|V|}_{i=0}I^v_i + \sum\limits^{|S|}_{j=0}I^s_j - I_{max})
% \label{eq:overall_suspicion_score}
% \end{equation}
% The overall suspicion score reflects the relative difference between the highest suspicion score and the average suspicion score of other elements. The underlying intuition is that for poisoned samples, the trigger's suspicion score (highest suspicion score) is significantly higher than the average suspicion score of normal elements. For normal samples, the suspicion score of the most vulnerable element is not markedly different from the average suspicion score of other normal elements. The right sub-figure in Figure \ref{fig:motivation} (b) supports this intuition, illustrating that the overall suspicion score distribution of poisoned samples is distinguishable from that of clean samples. We determine a sample with an overall suspicion score larger than $t$ (i.e., $OI > t$) as a poisoned sample and purify it by substituting the element with the highest suspicion score. The threshold $t$ can be tuned on normal samples (e.g., a validation set) to balance the performance of defense and semantic preservation.



\subsection{Purified Code Generation}
This step aims to purify the identified poisoned code by generating the substitution for the suspicious trigger using a masked language model that can be any code models having ``infilling'' capabilities, such as such as CodeBERT \cite{}, InCoder \cite{}, and ChatGPT \cite{}. For the sake of simplicity but without any loss of generality, the masked language model is exemplified by CodeBERT in this study. Specifically, CodeBERT employs Masked Language Modeling (MLM) \cite{} as its training objective, which is to predict the original tokens which are masked out. The MLM training objective enables us to directly use CodeBERT recover the tokens in place of the masked suspicious tokens in a zero-shot learning setting. The purification process via a masked language model $MLM$ can be formulated as:
\begin{equation}
X^{purified}_i = MLM(X^{masked}_i)
\end{equation}
With the purified code $X^{purified}_i$, we can make prediction using the victim model:
\begin{equation}
Y^{pre}_i = M(X^{purified}_i)
\end{equation}

==> sec/todo.tex <==
0. figure 2
1. website
2. citation
3. proof reading

==> sec/website.tex <==
% https://github.com/codepurify24/codepurify
% account elloworl620@gmail.com 
% password code_purify_2024

==> tab/rq1.tex <==
\begin{table*}[htbp]
\caption{RQ1.}
\label{tab:rq1}
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|c} 
\toprule
\multirow{2}{*}{Attacks} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}BNC\\(Fixed)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}BNC\\(Grammar)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}CodePoisoner\\(Deadcode)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}CodePoisoner\\(Variable)\end{tabular}} & \multirow{2}{*}{Average}  \\
                         & a=5\%                  & a=1\%                                            & a=5\%                  & a=1\%                                              & a=5\%                  & a=1\%                                                        & a=5\%                  & a=1\%                                                        &                           \\ 
\hline \hline
\multicolumn{10}{c}{{\cellcolor[rgb]{0.902,0.902,0.902}}Defect Detection}                                                                                                                                                                                                                                                                                                                      \\ 
\hline
CodeBERT                 & 100                    & 99.84                                            & 100                    & 100                                                & 100                    & 100                                                          & 100                    & 99.52                                                        & 99.92                     \\
~ +SS                    & 54.58                  & 59.04                                            & 61.59                  & 80.80                                              & 50.52                  & 98.96                                                        & 63.51                  & 54.82                                                        & 65.48                     \\ 
~ +AC                    & 72.99                  & 67.01                                            & 65.26                  & 65.82                                              & 61.67                  & 71.47                                                        & 71.79                  & 78.96                                                        & 69.37                     \\
~ +ONION                 & 72.27                  & 66.77                                            & 74.90                  & 76.57                                              & 65.50                  & 61.43                                                        & 94.66                  & 83.47                                                        & 74.45                     \\
~ +Ours                  & \textcolor{red}{36.33} & \textcolor{red}{27.01}                           & \textcolor{red}{36.65} & \textcolor{red}{46.77}                             & \textcolor{red}{47.09} & \textcolor{red}{52.91}                                       & \textcolor{red}{57.69} & \textcolor{red}{49.48}                                       & \textcolor{red}{44.24}    \\ 
\hline
CodeT5                   & 100                    & 100                                              & 100                    & 100                                                & 100                    & 99.76                                                        & 100                    & 93.07                                                        & 99.10                     \\
~ +SS                    & 66.69                  & 52.19                                            & 65.02                  & 75.62                                              & 76.25                  & 81.59                                                        & 66.14                  & 71.79                                                        & 69.41                     \\
~ +AC                    & 83.59                  & 84.06                                            & 72.75                  & 82.55                                              & 99.92                  & 88.37                                                        & 79.76                  & 85.74                                                        & 84.59                     \\
~ +ONION                 & 54.74                  & 51.79                                            & 64.22                  & 55.78                                              & 67.73                  & 52.59                                                        & 93.39                  & 73.47                                                        & 64.21                     \\
~ +Ours                  & \textcolor{red}{2.95}  & \textcolor{red}{4.54}                            & \textcolor{red}{2.23}  & \textcolor{red}{5.26}                              & \textcolor{red}{1.27}  & \textcolor{red}{5.34}                                        & \textcolor{red}{1.51}  & \textcolor{red}{11.47}                                       & \textcolor{red}{4.32}     \\ 
\hline
\multicolumn{10}{c}{{\cellcolor[rgb]{0.902,0.902,0.902}}Clone Detection}                                                                                                                                                                                                                                                                                                                       \\ 
\hline
CodeBERT                 & 100                    & 100                                              & 100                    & 100                                                & 100                    & 100                                                          & 100                    & 100                                                          & 100                       \\
~ +SS                    & 100                    & 100                                              & 100                    & 100                                                & 100                    & 100                                                          & 100                    & 100                                                          & 100                       \\
~ +AC                    & 100                    & 100                                              & 100                    & 100                                                & 100                    & 100                                                          & 27.92                  & 100                                                          & 90.99                     \\
~ +ONION                 & 99.7                   & 99.62                                            & 96.91                  & 97.07                                              & 89.77                  & 90.52                                                        & 99.85                  & 99.85                                                        & 96.66                     \\
~ +Ours                  & \textcolor{red}{12.87} & \textcolor{red}{14.15}                           & \textcolor{red}{11.59} & \textcolor{red}{17.68}                             & \textcolor{red}{22.87} & \textcolor{red}{23.55}                                       & \textcolor{red}{21.22} & \textcolor{red}{19.94}                                       & \textcolor{red}{17.98}    \\ 
\hline
CodeT5                   & 100                    & 100                                              & 100                    & 100                                                & 100                    & 100                                                          & 100                    & 100                                                          & 100                       \\
~ +SS                    & 100                    & 100                                              & 100                    & 100                                                & 100                    & 100                                                          & 100                    & 100                                                          & 100                       \\
~ +AC                    & 100                    & 100                                              & 24.08                  & 100                                                & 100                    & 100                                                          & 21.82                  & 100                                                          & 80.74                     \\
~ +ONION                 & 96.69                  & 99.7                                             & 97.07                  & 96.76                                              & 93.75                  & 88.64                                                        & 91.85                  & 99.92                                                        & 95.55                     \\
~ +Ours                  & \textcolor{red}{16.55} & \textcolor{red}{11.74}                           & \textcolor{red}{19.86} & \textcolor{red}{16.33}                             & \textcolor{red}{19.86} & \textcolor{red}{18.36}                                       & \textcolor{red}{17.38} & \textcolor{red}{14.82}                                       & \textcolor{red}{16.86}    \\ 
\hline
\multicolumn{10}{c}{{\cellcolor[rgb]{0.902,0.902,0.902}}Program Repair}                                                                                                                                                                                                                                                                                                                        \\ 
\hline
CodeBERT                 & 98.06                  & 100                                              & 100                    & 98.17                                              & 100                    & 100                                                          & 100                    & 100                                                          & 99.53                     \\
~ +SS                    & 97.83                  & 98.29                                            & 97.83                  & 98.06                                              & 97.94                  & 98.17                                                        & 4.91                   & 6.06                                                         & 74.89                     \\
~ +AC                    & 1.26                   & 1.37                                             & \textcolor{red}{1.26}  & 97.94                                              & 1.60                   & \textcolor{red}{1.26}                                        & \textcolor{red}{0}     & 12.11                                                        & 14.60                     \\
~ +ONION                 & 50.06                  & 52.57                                            & 41.94                  & 39.66                                              & 23.89                  & 24.57                                                        & 74.40                  & 73.83                                                        & 47.62                     \\
~ +Ours                  & \textcolor{red}{0.46}  & \textcolor{red}{0.46}                            & 3.20                   & \textcolor{red}{2.97}                              & \textcolor{red}{0.69}  & \textcolor{red}{1.26}                                        & 4.11                   & \textcolor{red}{5.94}                                        & \textcolor{red}{2.39}     \\ 
\hline
CodeT5                   & 98.17                  & 97.71                                            & 98.06                  & 97.83                                              & 100                    & 100                                                          & 100                    & 100                                                          & 98.97                     \\
~ +SS                    & 97.71                  & 97.71                                            & 97.37                  & 97.83                                              & 97.03                  & 96.00                                                        & \textcolor{red}{0}     & \textcolor{red}{0}                                           & 72.96                     \\
~ +AC                    & 1.14                   & \textcolor{red}{1.26}                            & 1.37                   & 97.37                                              & \textcolor{red}{0}     & \textcolor{red}{1.37}                                        & \textcolor{red}{0}     & 14.90                                                        & 14.68                     \\
~ +ONION                 & 54.40                  & 53.14                                            & 68.57                  & 66.17                                              & 47.31                  & 39.09                                                        & 74.51                  & 74.40                                                        & 59.70                     \\
~ +Ours                  & \textcolor{red}{0.69}  & 1.40                                             & \textcolor{red}{1.14}  & \textcolor{red}{3.09}                              & 0.80                   & 2.29                                                         & 5.83                   & 5.26                                                         & \textcolor{red}{2.56}     \\
\bottomrule
\end{tabular}
% }
\end{table*}

==> tab/rq1_v2.tex <==
\begin{table*}[thbp]
\centering
\caption{The ASR\textsubscript{D} (\%) of defense methods against various backdoor attacks. \textit{None} indicates no defense applied. Lower ASR\textsubscript{D} values indicate more effective defense methods. The best and second-best results are highlighted in bold and underlined.}
\label{tab:rq1}
\resizebox{0.72\textwidth}{!}{
\begin{tabular}{c|c|cc|cc|cc|cc|c} 
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Defense}                 & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}BNC\\(Fixed)\end{tabular}}             & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}BNC\\(Grammar)\end{tabular}}           & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}CodePoisoner\\(Dead-code)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}CodePoisoner\\(Variable)\end{tabular}} & \multirow{2}{*}{Average}                   \\
                              &                                          & $\alpha$=5\%                                     & $\alpha$=1\%                                     & $\alpha$=5\%                                     & $\alpha$=1\%                                     & $\alpha$=5\%                                   & $\alpha$=1\%                                       & $\alpha$=5\%                                   & $\alpha$=1\%                                       &                                            \\ 
\hline\hline
\multicolumn{11}{c}{Defect Detection}                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ 
\hline
\multirow{5}{*}{CodeBERT}     & {\cellcolor[rgb]{0.875,0.875,0.875}}None & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}99.84 & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100 & {\cellcolor[rgb]{0.875,0.875,0.875}}100     & {\cellcolor[rgb]{0.875,0.875,0.875}}100 & {\cellcolor[rgb]{0.875,0.875,0.875}}99.52   & {\cellcolor[rgb]{0.875,0.875,0.875}}99.92  \\
                              & SS                                       & \uline{54.58}                             & \uline{59.04}                             & \uline{61.59}                             & 80.80                                     & \uline{50.52}                           & 98.96                                       & \uline{63.51}                           & \uline{54.82}                               & \uline{65.48}                              \\
                              & AC                                       & 72.99                                     & 67.01                                     & 65.26                                     & \uline{65.82}                             & 61.67                                   & 71.47                                       & 71.79                                   & 78.96                                       & 69.37                                      \\
                              & ONION                                    & 72.27                                     & 66.77                                     & 74.90                                     & 76.57                                     & 65.50                                   & \uline{61.43}                               & 94.66                                   & 83.47                                       & 74.45                                      \\
                              & {\tool}                                     & \textbf{36.33}                            & \textbf{27.01}                            & \textbf{36.65}                            & \textbf{46.77}                            & \textbf{47.09}                          & \textbf{52.91}                              & \textbf{57.69}                          & \textbf{49.48}                              & \textbf{44.24}                             \\ 
\hline
\multirow{5}{*}{CodeT5}       & {\cellcolor[rgb]{0.875,0.875,0.875}}None & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100 & {\cellcolor[rgb]{0.875,0.875,0.875}}99.76   & {\cellcolor[rgb]{0.875,0.875,0.875}}100 & {\cellcolor[rgb]{0.875,0.875,0.875}}93.07   & {\cellcolor[rgb]{0.875,0.875,0.875}}99.10  \\
                              & SS                                       & 66.69                                     & 52.19                                     & 65.02                                     & 75.62                                     & 76.25                                   & 81.59                                       & \uline{66.14}                           & \uline{71.79}                               & 69.41                                      \\
                              & AC                                       & 83.59                                     & 84.06                                     & 72.75                                     & 82.55                                     & 99.92                                   & 88.37                                       & 79.76                                   & 85.74                                       & 84.59                                      \\
                              & ONION                                    & \uline{54.74}                             & \uline{51.79}                             & \uline{64.22}                             & \uline{55.78}                             & \uline{67.73}                           & \uline{52.59}                               & 93.39                                   & 73.47                                       & \uline{64.21}                              \\
                              & {\tool}                                     & \textbf{2.95}                             & \textbf{4.54}                             & \textbf{2.23}                             & \textbf{5.26}                             & \textbf{1.27}                           & \textbf{5.34}                               & \textbf{1.51}                           & \textbf{11.47}                              & \textbf{4.32}                              \\ 
\hline\hline
\multicolumn{11}{c}{Clone Detection}                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ 
\hline
\multirow{5}{*}{CodeBERT}     & {\cellcolor[rgb]{0.875,0.875,0.875}}None & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100 & {\cellcolor[rgb]{0.875,0.875,0.875}}100     & {\cellcolor[rgb]{0.875,0.875,0.875}}100 & {\cellcolor[rgb]{0.875,0.875,0.875}}100     & {\cellcolor[rgb]{0.875,0.875,0.875}}100    \\
                              & SS                                       & 100                                       & 100                                       & 100                                       & 100                                       & 100                                     & 100                                         & 100                                     & 100                                         & 100                                        \\
                              & AC                                       & 100                                       & 100                                       & 100                                       & 100                                       & 100                                     & 100                                         & \uline{27.92}                           & 100                                         & \uline{90.99}                              \\
                              & ONION                                    & \uline{99.7}                              & \uline{99.62}                             & \uline{96.91}                             & \uline{97.07}                             & \uline{89.77}                           & \uline{90.52}                               & 99.85                                   & \uline{99.85}                               & 96.66                                      \\
                              & {\tool}                                     & \textbf{12.87}                            & \textbf{14.15}                            & \textbf{11.59}                            & \textbf{17.68}                            & \textbf{22.87}                          & \textbf{23.55}                              & \textbf{21.22}                          & \textbf{19.94}                              & \textbf{17.98}                             \\ 
\hline
\multirow{5}{*}{CodeT5}       & {\cellcolor[rgb]{0.875,0.875,0.875}}None & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100 & {\cellcolor[rgb]{0.875,0.875,0.875}}100     & {\cellcolor[rgb]{0.875,0.875,0.875}}100 & {\cellcolor[rgb]{0.875,0.875,0.875}}100     & {\cellcolor[rgb]{0.875,0.875,0.875}}100    \\
                              & SS                                       & 100                                       & 100                                       & 100                                       & 100                                       & 100                                     & 100                                         & 100                                     & 100                                         & 100                                        \\
                              & AC                                       & 100                                       & 100                                       & \uline{24.08}                             & 100                                       & 100                                     & 100                                         & \uline{21.82}                           & 100                                         & \uline{80.74}                              \\
                              & ONION                                    & \uline{96.69}                             & \uline{99.7}                              & 97.07                                     & \uline{96.76}                             & \uline{93.75}                           & \uline{88.64}                               & 91.85                                   & \uline{99.92}                               & 95.55                                      \\
                              & {\tool}                                     & \textbf{16.55}                            & \textbf{11.74}                            & \textbf{19.86}                            & \textbf{16.33}                            & \textbf{19.86}                          & \textbf{18.36}                              & \textbf{17.38}                          & \textbf{14.82}                              & \textbf{16.86}                             \\ 
\hline\hline
\multicolumn{11}{c}{Program Repair}                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ 
\hline
\multirow{5}{*}{CodeBERT}     & {\cellcolor[rgb]{0.875,0.875,0.875}}None & {\cellcolor[rgb]{0.875,0.875,0.875}}98.06 & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}100   & {\cellcolor[rgb]{0.875,0.875,0.875}}98.17 & {\cellcolor[rgb]{0.875,0.875,0.875}}100 & {\cellcolor[rgb]{0.875,0.875,0.875}}100     & {\cellcolor[rgb]{0.875,0.875,0.875}}100 & {\cellcolor[rgb]{0.875,0.875,0.875}}100     & {\cellcolor[rgb]{0.875,0.875,0.875}}99.53  \\
                              & SS                                       & 97.83                                     & 98.29                                     & 97.83                                     & 98.06                                     & 97.94                                   & 98.17                                       & 4.91                                    & \uline{6.06}                                & 74.89                                      \\
                              & AC                                       & \uline{1.26}                              & \uline{1.37}                              & \textbf{1.26}                             & 97.94                                     & \uline{1.60}                            & \textbf{1.26}                               & \textbf{0}                              & 12.11                                       & \uline{14.60}                              \\
                              & ONION                                    & 50.06                                     & 52.57                                     & 41.94                                     & \uline{39.66}                             & 23.89                                   & \uline{24.57}                               & 74.40                                   & 73.83                                       & 47.62                                      \\
                              & {\tool}                                     & \textbf{0.46}                             & \textbf{0.46}                             & \uline{3.20}                              & \textbf{2.97}                             & \textbf{0.69}                           & \textbf{1.26}                               & \uline{4.11}                            & \textbf{5.94}                               & \textbf{2.39}                              \\ 
\hline
\multirow{5}{*}{CodeT5}       & {\cellcolor[rgb]{0.875,0.875,0.875}}None & {\cellcolor[rgb]{0.875,0.875,0.875}}98.17 & {\cellcolor[rgb]{0.875,0.875,0.875}}97.71 & {\cellcolor[rgb]{0.875,0.875,0.875}}98.06 & {\cellcolor[rgb]{0.875,0.875,0.875}}97.83 & {\cellcolor[rgb]{0.875,0.875,0.875}}100 & {\cellcolor[rgb]{0.875,0.875,0.875}}100     & {\cellcolor[rgb]{0.875,0.875,0.875}}100 & {\cellcolor[rgb]{0.875,0.875,0.875}}100     & {\cellcolor[rgb]{0.875,0.875,0.875}}98.97  \\
                              & SS                                       & 97.71                                     & 97.71                                     & 97.37                                     & 97.83                                     & 97.03                                   & 96.00                                       & \textbf{0}                              & \textbf{0}                                  & 72.96                                      \\
                              & AC                                       & \uline{1.14}                              & \textbf{1.26}                             & \uline{1.37}                              & 97.37                                     & \textbf{0}                              & \textbf{1.37}                               & \textbf{0}                              & 14.90                                       & \uline{14.68}                              \\
                              & ONION                                    & 54.40                                     & 53.14                                     & 68.57                                     & \uline{66.17}                             & 47.31                                   & 39.09                                       & 74.51                                   & 74.40                                       & 59.70                                      \\
                              & {\tool}                                     & \textbf{0.69}                             & \uline{1.40}                              & \textbf{1.14}                             & \textbf{3.09}                             & \uline{0.80}                            & \uline{2.29}                                & \uline{5.83}                            & \uline{5.26}                                & \textbf{2.56}                              \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tab/rq2.tex <==
\begin{table*}[htbp]
\caption{RQ2.}
\label{tab:my-table}
\begin{tabular}{l|cc|cc|cc|cc|c} 
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Attacks}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}BNC\\(Fixed)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}BNC\\(Grammar)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}CodePoisoner\\(Deadcode)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}CodePoisoner\\(Variable)\end{tabular}} & \multirow{2}{*}{Average}  \\
\multicolumn{1}{c|}{}                         & a=5\%                  & a=1\%                                            & a=5\%                  & a=1\%                                              & a=5\%                  & a=1\%                                                        & a=5\%                  & a=1\%                                                        &                           \\ 
\hline\hline
\multicolumn{10}{c}{{\cellcolor[rgb]{0.902,0.902,0.902}}Defect Detection}                                                                                                                                                                                                                                                                                                                                           \\ 
\hline
CodeBERT                                      & 61.38                  & 62.15                                            & 62.88                  & 63.65                                              & 62.63                  & 62.66                                                        & 62.45                  & 62.33                                                        & 62.52                     \\
~+SS                                          & \textcolor{red}{62.88} & \textcolor{red}{63.51}                           & 62.41                  & 62.77                                              & 62.11                  & \textcolor{red}{63.40}                                       & \textcolor{red}{61.82} & 62.19                                                        & \textcolor{red}{62.64}    \\
~+AC                                          & 56.70                  & 56.08                                            & 59.22                  & 57.65                                              & 58.38                  & 55.23                                                        & 59.85                  & 56.27                                                        & 57.42                     \\
~+ONION                                       & 58.49                  & 57.32                                            & 58.75                  & 57.65                                              & 58.86                  & 57.83                                                        & 57.14                  & 58.16                                                        & 58.03                     \\
~+Ours                                        & 61.27                  & 62.15                                            & \textcolor{red}{62.88} & \textcolor{red}{62.96}                             & \textcolor{red}{62.37} & 62.66                                                        & 61.68                  & \textcolor{red}{62.33}                                       & 62.29                     \\ 
\hline
CodeT5                                        & 60.21                  & 60.47                                            & 60.32                  & 58.67                                              & 61.42                  & 62.19                                                        & 61.60                  & 59.44                                                        & 60.54                     \\
~+SS                                          & 59.19                  & 59.48                                            & 60.14                  & \textcolor{red}{61.60}                             & 59.30                  & \textcolor{red}{61.24}                                       & 59.55                  & \textcolor{red}{60.72}                                       & \textcolor{red}{60.15}    \\
~+AC                                          & 56.48                  & 56.88                                            & 56.63                  & 56.88                                              & 50.04                  & 56.59                                                        & 58.57                  & 56.88                                                        & 56.12                     \\
~+ONION                                       & 56.03                  & 56.66                                            & 58.78                  & 56.52                                              & 57.65                  & 53.62                                                        & 57.17                  & 54.87                                                        & 56.41                     \\
~+Ours                                        & \textcolor{red}{60.18} & \textcolor{red}{59.77}                           & \textcolor{red}{60.25} & 58.38                                              & \textcolor{red}{61.38} & 58.71                                                        & \textcolor{red}{61.53} & 56.30                                                        & 59.56                     \\ 
\hline
\multicolumn{10}{c}{{\cellcolor[rgb]{0.902,0.902,0.902}}Clone Detection}                                                                                                                                                                                                                                                                                                                                            \\ 
\hline
CodeBERT                                      & 97.09                  & 96.96                                            & 97.31                  & 97.02                                              & 96.98                  & 96.57                                                        & 96.73                  & 96.79                                                        & 96.93                     \\
~+SS                                          & 96.41                  & \textcolor{red}{96.82}                           & 96.41                  & \textcolor{red}{97.09}                             & 96.42                  & \textcolor{red}{96.88}                                       & 96.15                  & 95.95                                                        & 96.52                     \\
~+AC                                          & 92.04                  & 92.51                                            & 94.86                  & 94.41                                              & 94.81                  & 94.89                                                        & 94.79                  & 88.01                                                        & 93.29                     \\
~+ONION                                       & 96.45                  & 95.6                                             & 95.72                  & 94.86                                              & 96.05                  & 96.53                                                        & 95.25                  & 96.48                                                        & 95.87                     \\
~+Ours                                        & \textcolor{red}{97.02} & 96.25                                            & \textcolor{red}{97.11} & 96.59                                              & \textcolor{red}{96.90} & 95.93                                                        & \textcolor{red}{96.64} & \textcolor{red}{96.54}                                       & \textcolor{red}{96.62}    \\ 
\hline
CodeT5                                        & 97.37                  & 97.40                                            & 97.16                  & 97.36                                              & 97.47                  & 97.51                                                        & 97.16                  & 97.01                                                        & 97.31                     \\
~+SS                                          & \textcolor{red}{96.89} & \textcolor{red}{97.25}                           & \textcolor{red}{96.85} & \textcolor{red}{97.40}                             & \textcolor{red}{97.51} & \textcolor{red}{97.03}                                       & \textcolor{red}{97.11} & \textcolor{red}{97.06}                                       & \textcolor{red}{97.14}    \\
~+AC                                          & 88.71                  & 92.71                                            & 95.41                  & 93.71                                              & 95.18                  & 94.60                                                        & 95.45                  & 88.27                                                        & 93.01                     \\
~+ONION                                       & 96.33                  & 97.25                                            & 97.02                  & 95.38                                              & 96.13                  & 96.28                                                        & 95.00                  & 95.20                                                        & 96.07                     \\
~+Ours                                        & 95.72                  & 95.85                                            & 95.09                  & 96.32                                              & 95.55                  & 96.7                                                         & 95.12                  & 96.20                                                        & 95.82                     \\ 
\hline
\multicolumn{10}{c}{{\cellcolor[rgb]{0.902,0.902,0.902}}Program Repair}                                                                                                                                                                                                                                                                                                                                             \\ 
\hline
CodeBERT                                      & 83.54                  & 83.57                                            & 82.84                  & 83.44                                              & 83.58                  & 82.89                                                        & 83.44                  & 83.02                                                        & 83.29                     \\
~+SS                                          & 83.08                  & \textcolor{red}{83.37}                           & \textcolor{red}{83.20} & 83.10                                              & 83.40                  & \textcolor{red}{83.52}                                       & 83.20                  & \textcolor{red}{83.44}                                       & \textcolor{red}{83.29}    \\
~+AC                                          & 82.37                  & 82.36                                            & 82.94                  & 83.21                                              & 83.31                  & 83.09                                                        & 83.09                  & 83.32                                                        & 82.96                     \\
~+ONION                                       & 46.45                  & 47.27                                            & 49.24                  & 50.5                                               & 47.06                  & 46.45                                                        & 46.72                  & 48.39                                                        & 47.76                     \\
~+Ours                                        & \textcolor{red}{83.36} & \textcolor{red}{83.37}                           & 82.78                  & \textcolor{red}{83.31}                             & \textcolor{red}{83.48} & 82.67                                                        & \textcolor{red}{83.28} & 82.90                                                        & 83.14                     \\ 
\hline
CodeT5                                        & 83.54                  & 83.64                                            & 83.57                  & 83.62                                              & 83.50                  & 83.61                                                        & 83.64                  & 83.58                                                        & 83.59                     \\
~+SS                                          & \textcolor{red}{83.58} & \textcolor{red}{83.61}                           & \textcolor{red}{83.71} & \textcolor{red}{83.69}                             & \textcolor{red}{83.47} & \textcolor{red}{83.63}                                       & \textcolor{red}{83.61} & \textcolor{red}{83.48}                                       & \textcolor{red}{83.60}    \\
~+AC                                          & 83.55                  & 83.74                                            & 83.67                  & 83.56                                              & 83.45                  & 83.49                                                        & 83.63                  & 83.57                                                        & 83.58                     \\
~+ONION                                       & 57.43                  & 57.56                                            & 57.85                  & 57.12                                              & 57.23                  & 56.82                                                        & 58.14                  & 57.28                                                        & 57.43                     \\
~+Ours                                        & 83.43                  & 83.50                                            & 83.51                  & 83.48                                              & 83.35                  & 83.44                                                        & 83.42                  & 83.46                                                        & 83.45                     \\
\bottomrule
\end{tabular}
\end{table*}

==> tab/rq2_v2.tex <==
\begin{table*}[htbp]
% \vspace{-0.3cm}
\centering
\caption{The performance of the victim models on the clean samples when employing different defense methods. For defect detection and clone detection tasks, we report ACC\textsubscript{D} (\%); for program repair task, the performance of BLEU\textsubscript{D} (\%) is reported. \textit{None} indicates no defense applied. Higher ACC\textsubscript{D} or BLEU\textsubscript{D} indicate more effective defense methods. The best and second-best results are highlighted in bold and underlined.}
\label{tab:rq2}
\vspace{-0.3cm}
\resizebox{0.71\textwidth}{!}{
\begin{tabular}{c|c|cc|cc|cc|cc|c} 
\toprule
\multirow{2}{*}{Model}    & \multirow{2}{*}{Defense}                 & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}BNC\\(Fixed)\end{tabular}}             & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}BNC\\(Grammar)\end{tabular}}           & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}CodePoisoner\\(Dead-code)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}CodePoisoner\\(Variable)\end{tabular}} & \multirow{2}{*}{Average}                   \\
                          &                                          & $\alpha$=5\%                                     & $\alpha$=1\%                                     & $\alpha$=5\%                                     & $\alpha$=1\%                                     & $\alpha$=5\%                                     & $\alpha$=1\%                                     & $\alpha$=5\%                                     & $\alpha$=1\%                                     &                                            \\ 
\hline\hline
\multicolumn{1}{c}{}      & \multicolumn{10}{c}{Defect Detection}                                                                                                                                                                                                                                                                                                                                                                                                                 \\ 
\hline
\multirow{5}{*}{CodeBERT} & {\cellcolor[rgb]{0.875,0.875,0.875}}None & {\cellcolor[rgb]{0.875,0.875,0.875}}61.38 & {\cellcolor[rgb]{0.875,0.875,0.875}}62.15 & {\cellcolor[rgb]{0.875,0.875,0.875}}62.88 & {\cellcolor[rgb]{0.875,0.875,0.875}}63.65 & {\cellcolor[rgb]{0.875,0.875,0.875}}62.63 & {\cellcolor[rgb]{0.875,0.875,0.875}}62.66 & {\cellcolor[rgb]{0.875,0.875,0.875}}62.45 & {\cellcolor[rgb]{0.875,0.875,0.875}}62.33 & {\cellcolor[rgb]{0.875,0.875,0.875}}62.52  \\
                          & SS                                       & \textbf{62.88}                            & \textbf{63.51}                            & \uline{62.41}                             & \uline{62.77}                             & \uline{62.11}                             & \textbf{63.40}                            & \textbf{61.82}                            & \uline{62.19}                             & \textbf{62.64}                             \\
                          & AC                                       & 56.70                                     & 56.08                                     & 59.22                                     & 57.65                                     & 58.38                                     & 55.23                                     & 59.85                                     & 56.27                                     & 57.42                                      \\
                          & ONION                                    & 58.49                                     & 57.32                                     & 58.75                                     & 57.65                                     & 58.86                                     & 57.83                                     & 57.14                                     & 58.16                                     & 58.03                                      \\
                          & {\tool}                                     & \uline{61.27}                             & \uline{62.15}                             & \textbf{62.88}                            & \textbf{62.96}                            & \textbf{62.37}                            & \uline{62.66}                             & \uline{61.68}                             & \textbf{62.33}                            & \uline{62.29}                              \\ 
\hline
\multirow{5}{*}{CodeT5}   & {\cellcolor[rgb]{0.875,0.875,0.875}}None & {\cellcolor[rgb]{0.875,0.875,0.875}}60.21 & {\cellcolor[rgb]{0.875,0.875,0.875}}60.47 & {\cellcolor[rgb]{0.875,0.875,0.875}}60.32 & {\cellcolor[rgb]{0.875,0.875,0.875}}58.67 & {\cellcolor[rgb]{0.875,0.875,0.875}}61.42 & {\cellcolor[rgb]{0.875,0.875,0.875}}62.19 & {\cellcolor[rgb]{0.875,0.875,0.875}}61.60 & {\cellcolor[rgb]{0.875,0.875,0.875}}59.44 & {\cellcolor[rgb]{0.875,0.875,0.875}}60.54  \\
                          & SS                                       & \uline{59.19}                             & \uline{59.48}                             & \uline{60.14}                             & \textbf{61.60}                            & \uline{59.30}                             & \textbf{61.24}                            & \uline{59.55}                             & \textbf{60.72}                            & \textbf{60.15}                             \\
                          & AC                                       & 56.48                                     & 56.88                                     & 56.63                                     & 56.88                                     & 50.04                                     & 56.59                                     & 58.57                                     & \uline{56.88}                             & 56.12                                      \\
                          & ONION                                    & 56.03                                     & 56.66                                     & 58.78                                     & 56.52                                     & 57.65                                     & 53.62                                     & 57.17                                     & 54.87                                     & 56.41                                      \\
                          & {\tool}                                     & \textbf{60.18}                            & \textbf{59.77}                            & \textbf{60.25}                            & \uline{58.38}                             & \textbf{61.38}                            & \uline{58.71}                             & \textbf{61.53}                            & 56.30                                     & \uline{59.56}                              \\ 
\hline\hline
\multicolumn{11}{c}{Clone Detection}                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ 
\hline
\multirow{5}{*}{CodeBERT} & {\cellcolor[rgb]{0.875,0.875,0.875}}None & {\cellcolor[rgb]{0.875,0.875,0.875}}97.09 & {\cellcolor[rgb]{0.875,0.875,0.875}}96.96 & {\cellcolor[rgb]{0.875,0.875,0.875}}97.31 & {\cellcolor[rgb]{0.875,0.875,0.875}}97.02 & {\cellcolor[rgb]{0.875,0.875,0.875}}96.98 & {\cellcolor[rgb]{0.875,0.875,0.875}}96.57 & {\cellcolor[rgb]{0.875,0.875,0.875}}96.73 & {\cellcolor[rgb]{0.875,0.875,0.875}}96.79 & {\cellcolor[rgb]{0.875,0.875,0.875}}96.93  \\
                          & SS                                       & 96.41                                     & \textbf{96.82}                            & \uline{96.41}                             & \textbf{97.09}                            & \uline{96.42}                             & \textbf{96.88}                            & \uline{96.15}                             & 95.95                                     & \uline{96.52}                              \\
                          & AC                                       & 92.04                                     & 92.51                                     & 94.86                                     & 94.41                                     & 94.81                                     & 94.89                                     & 94.79                                     & 88.01                                     & 93.29                                      \\
                          & ONION                                    & \uline{96.45}                             & 95.60                                     & 95.72                                     & 94.86                                     & 96.05                                     & \uline{96.53}                             & 95.25                                     & \uline{96.48}                             & 95.87                                      \\
                          & {\tool}                                     & \textbf{97.02}                            & \uline{96.25}                             & \textbf{97.11}                            & \uline{96.59}                             & \textbf{96.90}                            & 95.93                                     & \textbf{96.64}                            & \textbf{96.54}                            & \textbf{96.62}                             \\ 
\hline
\multirow{5}{*}{CodeT5}   & {\cellcolor[rgb]{0.875,0.875,0.875}}None & {\cellcolor[rgb]{0.875,0.875,0.875}}97.37 & {\cellcolor[rgb]{0.875,0.875,0.875}}97.40 & {\cellcolor[rgb]{0.875,0.875,0.875}}97.16 & {\cellcolor[rgb]{0.875,0.875,0.875}}97.36 & {\cellcolor[rgb]{0.875,0.875,0.875}}97.47 & {\cellcolor[rgb]{0.875,0.875,0.875}}97.51 & {\cellcolor[rgb]{0.875,0.875,0.875}}97.16 & {\cellcolor[rgb]{0.875,0.875,0.875}}97.01 & {\cellcolor[rgb]{0.875,0.875,0.875}}97.31  \\
                          & SS                                       & \textbf{96.89}                            & \textbf{97.25}                            & \textbf{96.85}                            & \textbf{97.40}                            & \textbf{97.51}                            & \textbf{97.03}                            & \textbf{97.11}                            & \textbf{97.06}                            & \textbf{97.14}                             \\
                          & AC                                       & 88.71                                     & 92.71                                     & 95.41                                     & 93.71                                     & 95.18                                     & 94.60                                     & \uline{95.45}                             & 88.27                                     & 93.01                                      \\
                          & ONION                                    & \uline{96.33}                             & \textbf{97.25}                            & \uline{97.02}                             & 95.38                                     & \uline{96.13}                             & 96.28                                     & 95.00                                     & 95.20                                     & \uline{96.07}                              \\
                          & {\tool}                                     & 95.72                                     & \uline{95.85}                             & 95.09                                     & \uline{96.32}                             & 95.55                                     & \uline{96.70}                             & 95.12                                     & \uline{96.20}                             & 95.82                                      \\ 
\hline\hline
\multicolumn{11}{c}{Program Repair}                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ 
\hline
\multirow{5}{*}{CodeBERT} & {\cellcolor[rgb]{0.875,0.875,0.875}}None & {\cellcolor[rgb]{0.875,0.875,0.875}}83.54 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.57 & {\cellcolor[rgb]{0.875,0.875,0.875}}82.84 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.44 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.58 & {\cellcolor[rgb]{0.875,0.875,0.875}}82.89 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.44 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.02 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.29  \\
                          & SS                                       & \uline{83.08}                             & \textbf{83.37}                            & \textbf{83.20}                            & 83.10                                     & \uline{83.40}                             & \textbf{83.52}                            & \uline{83.20}                             & \textbf{83.44}                            & \textbf{83.29}                             \\
                          & AC                                       & 82.37                                     & \uline{82.36}                             & \uline{82.94}                             & \uline{83.21}                             & 83.31                                     & \uline{83.09}                             & 83.09                                     & \uline{83.32}                             & 82.96                                      \\
                          & ONION                                    & 46.45                                     & 47.27                                     & 49.24                                     & 50.5                                      & 47.06                                     & 46.45                                     & 46.72                                     & 48.39                                     & 47.76                                      \\
                          & {\tool}                                     & \textbf{83.36}                            & \textbf{83.37}                            & 82.78                                     & \textbf{83.31}                            & \textbf{83.48}                            & 82.67                                     & \textbf{83.28}                            & 82.90                                     & \uline{83.14}                              \\ 
\hline
\multirow{5}{*}{CodeT5}   & {\cellcolor[rgb]{0.875,0.875,0.875}}None & {\cellcolor[rgb]{0.875,0.875,0.875}}83.54 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.64 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.57 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.62 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.50 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.61 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.64 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.58 & {\cellcolor[rgb]{0.875,0.875,0.875}}83.59  \\
                          & SS                                       & \textbf{83.58}                            & \textbf{83.61}                            & \textbf{83.71}                            & \textbf{83.69}                            & \textbf{83.47}                            & \textbf{83.63}                            & \textbf{83.61}                            & \textbf{83.48}                            & \textbf{83.60}                             \\
                          & AC                                       & \uline{83.55}                             & \uline{83.74}                             & \uline{83.67}                             & \uline{83.56}                             & \uline{83.45}                             & \uline{83.49}                             & \uline{83.63}                             & \uline{83.57}                             & \uline{83.58}                              \\
                          & ONION                                    & 57.43                                     & 57.56                                     & 57.85                                     & 57.12                                     & 57.23                                     & 56.82                                     & 58.14                                     & 57.28                                     & 57.43                                      \\
                          & {\tool}                                     & 83.43                                     & 83.50                                     & 83.51                                     & 83.48                                     & 83.35                                     & 83.44                                     & 83.42                                     & 83.46                                     & 83.45                                      \\
\bottomrule
\end{tabular}
\vspace{-0.6cm}
}
\end{table*}

==> tab/rq3.tex <==
\begin{table*}[hbtp!]
\centering
\caption{RQ3}
\label{table:rq1}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}clllllllll@{}}
\midrule
\multirow{2}{*}{Method}    & \multicolumn{3}{c}{Codex}      & \multicolumn{3}{c}{CodeGen}    & \multicolumn{3}{c}{Incoder}    \\ 
                           & LeetCode & HumanEval & DS-1000 & LeetCode & HumanEval & DS-1000 & LeetCode & HumanEval & DS-1000 \\ \hline
Original                   & 11.36\%         &   47.56\%        &   38.4\%      &   3.34\%       &   16.4\%        &  7.8\%      &  1.94\%        &    11.3\%       &  4.0\%       \\ 
Oracle                 &  26.59\%        &  72.56\%         &   57.4\%      &  13.37\%        &  24.4\%         &  19.6\%       & 3.06\%         &   24.7\%        &   12.7\%      \\ 
 Random                  &    10.52\%      &    46.95\%       &  38.1\%       &   3.06\%       &    15.2\%       &    7.2\%     &  1.11\%        &   10.4\%        &  4.5\%       \\ \hline
\rowcolor{gray!25}Ours  &  14.48 (26.83)\%        &   57.32 (20.51)\%        &   40.3(4.9)\%      &  3.89(8.33)\%        &  17.07(3.7)\%         & 10.0(28.2)\%        &   1.94(0)\%       & 13.4(22.2)\%          &  6.8(70)\%       \\
Ours w/o template  &   \%        &    \%        &    \%      &   \%        &   \%         & \%        &    \%       &  \%          &  \%       \\
Ours w/o n2c  &  11.36\%        &   49.39\%        &   38.4\%      &  3.34\%        &  12.8\%         & 8.9\%        &   1.39\%       & 12.8\%          &  6.3\%       \\
Ours w/o c2c  &  12.26\%        &   48.78\%        &   34.3\%      &  3.89\%        &  11.59\%         & 8.2\%        &   2.22\%       & 11.59\%          &  5.8\%       \\\bottomrule
\end{tabular}
}
\end{table*}
